LoRA Adaptation Strength in Aurora-WRF: Trade-offs in Regional Heavy-Rainfall Forecasting

We investigate how parameter-efficient adaptation of an atmospheric foundation model affects downstream regional precipitation in a controlled Aurora-WRF coupling experiment over the Beijing-Tianjin-Hebei region. A single-step, precipitation-weighted LoRA adaptation of AuroraPretrained is trained on May-September 2020-2021 and selected using 2022 validation data. Five inference-time adaptation strengths are coupled to an unchanged 9-km WRF configuration and compared with a GFS-driven control under common ERA5 initialization and auxiliary-field rules. Evaluation uses 17 initializations in 2023, hourly ERA5 precipitation, and conservative remapping to a fixed 356-cell, 0.25-degree verification grid. Heavy rainfall is defined exclusively as at least 50 mm in a continuous 24-hour window, advanced hourly. For window starts from 0 to 48 hours, unadapted Aurora attains the highest mean critical success index (CSI), 0.216, compared with 0.144 for the GFS control. An intermediate LoRA strength of 0.75 reduces the Aurora-driven 24-hour precipitation mean squared error by 30.7% and brings pooled frequency Bias from 1.510 to 1.024, but lowers CSI to 0.182. GFS retains the lowest whole-domain error. These results characterize a trade-off between rainfall detection, frequency calibration, and intensity error, showing the importance of evaluating adaptation strength against multiple downstream criteria within a common coupling framework.

==> tables/cases.tex <==
2023-05-07 & 0 & 0 & 0.23 \\
2023-05-15 & 6 & 1 & 51.00 \\
2023-05-21 & 0 & 0 & 2.01 \\
2023-06-03 & 0 & 0 & 1.12 \\
2023-06-14 & 0 & 0 & 1.36 \\
2023-06-26 & 0 & 0 & 47.92 \\
2023-07-02 & 112 & 6 & 63.43 \\
2023-07-10 & 252 & 19 & 92.59 \\
2023-07-20 & 1122 & 35 & 253.01 \\
2023-07-30 & 2624 & 147 & 211.49 \\
2023-08-07 & 0 & 0 & 17.48 \\
2023-08-10 & 857 & 43 & 91.47 \\
2023-08-19 & 108 & 8 & 73.08 \\
2023-08-21 & 0 & 0 & 41.10 \\
2023-08-25 & 12 & 1 & 56.67 \\
2023-09-01 & 0 & 0 & 22.74 \\
2023-09-07 & 498 & 32 & 89.92 \\


==> tables/dispersion.tex <==
GFS & $0.037 \pm 0.056$ (10) & $1.173 \pm 1.343$ (9) & $167.88 \pm 262.22$ (17) & $1.45 \pm 2.01$ (17) \\
$\alpha=0$ & $0.037 \pm 0.082$ (12) & $2.523 \pm 4.393$ (9) & $302.20 \pm 541.73$ (17) & $2.30 \pm 3.63$ (17) \\
$\alpha=0.25$ & $0.025 \pm 0.075$ (12) & $2.486 \pm 5.496$ (9) & $296.94 \pm 626.85$ (17) & $1.97 \pm 4.02$ (17) \\
$\alpha=0.50$ & $0.026 \pm 0.077$ (10) & $5.786 \pm 15.880$ (9) & $233.14 \pm 376.13$ (17) & $1.53 \pm 2.92$ (17) \\
$\alpha=0.75$ & $0.025 \pm 0.076$ (10) & $5.780 \pm 15.427$ (9) & $209.57 \pm 273.28$ (17) & $1.56 \pm 2.43$ (17) \\
$\alpha=1$ & $0.025 \pm 0.079$ (11) & $19.949 \pm 56.790$ (9) & $274.73 \pm 390.98$ (17) & $2.00 \pm 3.00$ (17) \\

==> tables/extended.tex <==
GFS & 0.101 & 70 & 0.996 & 128.57 \\
$\alpha=0$ & 0.145 & 73 & 1.704 & 240.74 \\
$\alpha=0.25$ & 0.136 & 73 & 1.672 & 260.23 \\
$\alpha=0.50$ & 0.129 & 73 & 1.498 & 205.56 \\
$\alpha=0.75$ & 0.122 & 73 & 1.284 & 181.77 \\
$\alpha=1$ & 0.121 & 73 & 2.201 & 257.70 \\

==> tables/main.tex <==
GFS & 0.144 & 0.896 & 0.218 & 0.757 & 5.17 & 167.88 \\
$\alpha=0$ & 0.216 & 1.510 & 0.405 & 0.732 & 7.16 & 302.20 \\
$\alpha=0.25$ & 0.202 & 1.326 & 0.332 & 0.749 & 6.81 & 296.94 \\
$\alpha=0.50$ & 0.192 & 1.131 & 0.305 & 0.730 & 6.40 & 233.14 \\
$\alpha=0.75$ & 0.182 & 1.024 & 0.286 & 0.720 & 6.47 & 209.57 \\
$\alpha=1$ & 0.180 & 1.649 & 0.327 & 0.802 & 7.01 & 274.73 \\
